A short proof of Allard's and Brakke's regularity theorems

We give new short proofs of Allard's regularity theorem for varifolds with bounded first variation and Brakke's regularity theorem for integral Brakke flows with bounded forcing. They are based on a decay of flatness, following from weighted versions of the respective monotonicity formulas, together with a characterization of non-homogeneous blow-ups using the viscosity approach introduced by Savin.

==> Commands0.tex <==
% ------------------------mathbb-----------------------------------
\newcommand{\RR}{{\mathbb R}}
\newcommand{\NN}{{\mathbb N}}


% ------------------------mathcal-----------------------------------
\renewcommand{\Mc}{\mathcal{M}}
%\newcommand{\Dc}{\mathcal{D}}
\newcommand{\Hc}{\mathcal{H}}


%-------------------------boldface-----------------------------------
\newcommand{\Mb}{\mathbf{M}}


% ------------------------Operators, arrows, similar--------------------
\newcommand{\weakly}{\rightharpoonup}
\newcommand{\graph}{\mathop{\rm graph}}
\newcommand{\compact}{\subset\subset}
\newcommand{\rest}{\llcorner}
\DeclareMathOperator{\supp}{supp}
\DeclareMathOperator{\dive}{div}

\renewcommand{\ge }{\geq}
\renewcommand{\le }{\leq}

\newcommand{\de}{\partial}
\newcommand{\compl}{c}			%COMPLEMENT OF A SET


%-------------------------Other letters--------------------------------
\newcommand{\eps}{\varepsilon}		%Renaming $\eps$
\let\oldphi\phi						%Replacing $\phi$ with $\varphi$ and keeping $\varphi$ in $\phin$
\newcommand{\phin}{\oldphi}
\renewcommand{\phi}{\varphi}


%-----------------------Accents-----------------------------------------
\renewcommand{\hat }{\widehat}
\renewcommand{\tilde }{\widetilde}

%------------------Other commands, specific -----------
\newcommand{\hk}{\Psi}			%heat kernel
\DeclareMathOperator{\Clos}{Clos}		%Closure of a set
\newcommand{\Gr}{\mathrm{Gr}}	%Grassmanian 

\DeclareMathOperator{\osc}{osc} 	%Oscillations
%\renewcommand{\flat}{\operatorname{flat}} 	%Flatness

\newcommand{\tSigma}{\tilde\Sigma}  %Rescalings of the support

\newcommand{\hhk}{\hat\hk}	%truncated heat kernel
\newcommand{\Var}[1]{V_{{#1}}}	%Varifolds

\newcommand{\dif}{\mathop{}\!\mathrm{d}}	%Differentials
\newcommand{\holder}{H\"{o}lder}
\newcommand{\trace}{\mathrm{trace}}

\newcommand{\Id}{\mathbbm{1}}
\newcommand{\transp}{\mathsf{T}}
